Beyond the Pixel-Wise Loss for Topology-Aware Delineation

Delineation of curvilinear structures is an important problem in Computer Vision with multiple practical applications. With the advent of Deep Learning, many current approaches on automatic delineation have focused on finding more powerful deep architectures, but have continued using the habitual pixel-wise losses such as binary cross-entropy. In this paper we claim that pixel-wise losses alone are unsuitable for this problem because of their inability to reflect the topological impact of mistakes in the final prediction. We propose a new loss term that is aware of the higher-order topological features of linear structures. We also introduce a refinement pipeline that iteratively applies the same model over the previous delineation to refine the predictions at each step while keeping the number of parameters and the complexity of the model constant. When combined with the standard pixel-wise loss, both our new loss term and our iterative refinement boost the quality of the predicted delineations, in some cases almost doubling the accuracy as compared to the same classifier trained with the binary cross-entropy alone. We show that our approach outperforms state-of-the-art methods on a wide range of data, from microscopy to aerial images.

==> fig/topology_loss_ag_copy.tex <==
\begin{figure*}[t]
  \centering
\begin{tabular}{ccccc}
  \includegraphics[width=0.17\textwidth]{fig/loss_example/orig.png} &
  \includegraphics[width=0.17\textwidth]{fig/loss_example/single_mistake.png} &
  \includegraphics[width=0.17\textwidth]{fig/loss_example/many_mistakes.png} &
  \includegraphics[width=0.17\textwidth]{fig/loss_example/single_cut.png} &
   \includegraphics[width=0.17\textwidth]{fig/loss_example/many_cuts.png}\\
        & $\bL_{top} = 0.2279$ & $\bL_{top} = 0.7795$ & $\bL_{top} = 0.2858$ & $\bL_{top} = 0.9977$\\
    (a)&(b)&(c)&(d)&(e)\\
\end{tabular}
  \caption{{\bf The effect of mistakes on topology loss.} {\small (a) Ground truth (b)-(e) we flip 240 pixels in each prediction, so that $\bL_{bce}$ is the same for all of them, but as we see $\bL_{top}$ penalizes more the cases with more small mistakes, which considerably change the structure of the prediction.}}
  \label{fig:topo_loss}
\end{figure*}


\begin{figure}
  \centering
\begin{tabular}{ccc}
  \hspace{-5mm} \includegraphics[width=0.16\textwidth]{fig/activations_example/gt.png} &
  \hspace{-4mm} \includegraphics[width=0.16\textwidth]{fig/activations_example/gt_act1.png} &
  \hspace{-4mm} \includegraphics[width=0.16\textwidth]{fig/activations_example/gt_act2.png} & \\
  \hspace{-5mm} \includegraphics[width=0.16\textwidth]{fig/activations_example/pred.png} &
  \hspace{-4mm} \includegraphics[width=0.16\textwidth]{fig/activations_example/pred_act1.png} &
  \hspace{-4mm} \includegraphics[width=0.16\textwidth]{fig/activations_example/pred_act2.png} & \\
  \hspace{-5mm} (a) & (b) & (c) \\
\end{tabular}
\vspace{-3mm}
  \caption{{\bf Examples of activations in VGG layers.} {\small (a) Ground-truth and corresponding prediction with errors. (b) Responses of a VGG19 channel specialized in elongated structures. (c) Responses of a VGG19 channel specialized in small connected components. $\bL_{top}$~strongly encourages responses in the former and penalizes responses in the latter.}}
  \label{fig:activations}
\end{figure}

